A Programming Language Oriented Approach to Computability

The field of computability and complexity was, where computer science sprung from. Turing, Church, and Kleene all developed formalisms that demonstrated what they held "intuitively computable". The times change however and today's (aspiring) computer scientists are less proficient in building automata or composing functions and are much more native to the world of programming languages. This article will try to introduce typical concepts of computability theory and complexity in a form more fitted for a modern developer. It is mostly based on \cite{jones}, but takes input from other sources to provide examples, additional information, etc.

==> abstract.tex <==
The field of computability and complexity was, where computer science
sprung from. Turing, Church, and Kleene all developed formalisms that
demonstrated what they held "intuitively computable". The times change
however and today's (aspiring) computer scientists are less proficient in
building automata or composing functions and are much more native to the
world of programming languages. This article will try to introduce typical
concepts of computability theory and complexity in a form more fitted for
a modern developer.  It is mostly based on \cite{jones}, but takes input
from other sources to provide examples, additional information, etc.

